HUGE: An Efficient and Scalable Subgraph Enumeration System

Subgraph enumeration is a fundamental problem in graph analytics, which aims to find all instances of a given query graph on a large data graph. In this paper, we propose a system called HUGE to efficiently process subgraph enumeration at scale in the distributed context. HUGE features 1) an optimiser to compute an advanced execution plan without the constraints of existing works; 2) a hybrid communication layer that supports both pushing and pulling communication; 3) a novel two-stage execution mode with a lock-free and zero-copy cache design, 4) a BFS/DFS-adaptive scheduler to bound memory consumption, and 5) two-layer intra- and inter-machine load balancing. HUGE is generic such that all existing distributed subgraph enumeration algorithms can be plugged in to enjoy automatic speed up and bounded-memory execution.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> contents/framework-old.tex <==
\section{The computation framework}
\label{sec:framework}

Different from all existing works \cite{crystaljoin,wco-join,twin-twig,edge-join,star-join,seed,psgl,RADS,BENU,multiway-join} that are coupled with certain execution plan (e.g. worst-case optimal, binary join etc.), \page engine generalizes the computation of subgraph enumeration in all existing works via a generic computation framework.

\subsection{Existing Approaches}



% The framework includes necessary \emph{operator}s and how to use them to represent different \emph{execution plan}s. 

% \begin{definition}
% An operator is the basic computing unit to schedule in \page. Each operator has a predefined computing logic, with a certain number of in-bound channels and out-bound channels to handle data input and output. An execution plan of subgraph enumeration is a directed tree structure, where the vertex stands for a \page operator, and the directed edges represents the data flow. Specifically, an edge from operators $O_1$ to $O_2$ in an execution plan means that the output of $O_1$ is the input of $O_2$. We call $O_1$ the \emph{precursor} of $O_2$, and $O_2$ the \emph{successor} of $O_1$.
% \end{definition}

% We list necessary concepts before presenting the \page engine:
% \begin{itemize}[leftmargin=*]
%     \item \emph{Operator}: An operator is the basic computing unit to schedule in \page. Each operator has a predefined computing logic, with a certain number of in-bound channels and out-bound channels to handle data input and output. 
%     \item \emph{Execution plan}: An execution plan of subgraph enumeration is a directed tree structure, where the vertex stands for a \page operator, and the directed edges represents the data flow. Specifically, an edge from operators $O_1$ to $O_2$ in an execution plan means that the output data of $O_1$ is the input data of $O_2$.
%     \item \emph{Micro-batch}: As a common practice of big data engines \cite{spark,storm,naiad} to fully utilize network resources, each operator in \page will process certain number of data as a batch at a time. Such minimum data processing unit is called a \emph{micro-batch} in the following. 
%     % We call a minimum  unit of an operator as a micro-batch, whose size is pre-configured by the users. Similar to many big data processing systems such as Spark \cite{spark}, the data in the in-bound channels is consumed batch by batch and the results are send to the out-bound channels.
% \end{itemize}

\subsection{Operators}
\label{sec:opt}

%Upon receiving an arbitrary execution plan, \page distributes the plan to every machine, executes it in parallel, and returns the results as needed. We have designed fundamental operators for \page to support different execution plans, as will be introduced below.

We introduce 4 primitive \page operators (\scan, \extend, \join, \sink) and 1 auxiliary operators (\clone) to represent subgraph enumeration plans. More operators can be added to \page to support complex analytical tasks on property graphs \cite{TinkerPop, neo4j}, which will be left as an interesting future work. 

%The core operators comprise essential operations for distributed subgraph enumeration, while auxiliary operators are designed for optimisation purpose. We describe each operator below.
% Keep this in mind, we should write in the sense that these are just operators that are necessary to understand this paper, while \page can support more operators. For example, to support Cypher queries while mentioning GraphFlow in the related work.

% Each operator in \page takes certain input steams (and/or the data graph) and produces typically one output stream when running inside the \page compute engine. \page operators adopt the well-known concept of \emph{micro-batch processing} for execution, similar to many streaming process systems such as Spark Streaming \cite{spark} and Timely Dataflow \cite{naiad}. 

% The input streams will be consumed and send to the output stream batch by batch to achieve a high throughput. We call each batch cycle of an operator a \emph{round}. Operators are scheduled and run inside the compute engine by multiple workers as discussed in \refsec{schedule}.

\stitle{SCAN.} The \scan operator takes a local partition of the data graph $G$ as its input, scans the partition, and computes sub-queries that can be independently enumerated within the local partition. Such sub-queries include edges and stars (a tree of depth $1$) as a practice from existing works \cite{star-join,twin-twig}. \scan is always the first operator of a valid execution plan as the data source. The \scan operator is abstracted as:

\centerline{\includegraphics{figures/scan.pdf}}

\stitle{JOIN.} \join operator is essential to support join-based subgraph enumeration plan. \join takes two input channels and performs a binary join based on the \emph{join key} and produce one single output channel.
% The implementation of a distributed join is given in \refsec{bd-join}. 
% We implemented the \join operator using local parallel hash join \cite{pjoin}.
% \join is usually used together with \exchange and \buffer to form a distributed join \cite{djoin}.

\centerline{\includegraphics{figures/join.pdf}}

\stitle{EXTEND.} Given partial results with each result in the form $p=\{u_1,u_2,\dots,u_k\}$, the \extend operator extends each partial result by one more vertex and produces an output channel containing of the extended results $p'=\{u_1,u_2,\dots,u_k,u_{k+1}\}$. An \emph{extend index}, $Ext=\{d_1,d_2,\dots,d_i\}$, is defined for each \extend operator, representing relevant vertices connected to the current extended vertex. Here, the set of $u_{k+1}$ is computed as the intersection of the neighbours of corresponding matched vertices $\bigcap_{i}^{n=0} \mathcal{N}_G(p[d_n])$. 
% The \extend operator is originally introduced in \cite{wco-join}, while
% We efficiently implement the \extend operator in the distributed environment using the pull-based scheme as will be detailed in \refsec{pull}. 
%\extend is the key for pull-based scheme that pulls remote vertices by calling the \nbrs RPC when necessary, and caches them accordingly. 
  %The implementation of \extend will be discussed in \refsec{pull}.

\centerline{\includegraphics{figures/extend.pdf}}

\stitle{SINK.} \sink is used to consume the results of subgraph enumeration. Typical sink procedures are to count the number of results or write the results (raw or compressed \cite{crystaljoin}) to disk.

%\stitle{Discussions.} \extend and \join are two operators that require communicating data via the network. For \extend, we adopt the pull-based scheme, as it only needs to retrieve the vertex data (neighbors)

\centerline{\includegraphics{figures/sink.pdf}}

% \stitle{EXCHANGE} \exchange intends to shuffle the data across machines in the cluster. In detail, it takes an input stream and calculates the hash value of each item in the stream using a built-in hash function $h$. An item $I$ is then routed to machine $h(I)\%k$ where $k$ is the total number of machines. In this paper, there are two scenarios that require \exchange. The first is to accomplish a distributed join followed by a \join operator. The second is to facilitate aggregating data (e.g. counting) for the \sink operator.
% The implementation details of \exchange connects a target machine with a TCP stream and send corresponding data in batches. 
% It is worth to mention that both of the two aforementioned scenarios require synchronization, so \exchange will wait until all machines in the cluster have completed the exchange process.

% \centerline{\includegraphics{figures/exchange.pdf}}

% \stitle{BUFFER} We can use the auxiliary operator \buffer to buffer intermediate results wherever it is possible to overflow the memory. \buffer takes an input streams and has a fixed size of in-memory space to buffer the stream it received. When the in-memory buffer is full, it spills them to the disk. \buffer will perform an optional \emph{external merge sort} if specified by the users and sort buffered results by built-in keys. If sorting is enabled, the data will be read back in the order of the keys. 
% As writing to and reading from disk are in-general costly, one may prefer an execution plan that are free from such operation.
% 
% \centerline{\includegraphics{figures/buffer.pdf}}

% \stitle{CLONE.} \clone is an auxiliary operator that takes a single input channel and produces two identical output channels by simply cloning one to another. A typical use case of \clone is to reuse the intermediate results of enumerating some partial queries to avoid duplicated computation.
% Additionally, \clone can be used together with \sink to save intermediate results to the disk as checkpoints to further improve the the system's reliability.

% \centerline{\includegraphics{figures/clone.pdf}}

\subsection{Execution Plan}
\label{sec:plan}
%There are intensive efforts in studying better execution plans for subgraph enumeration tasks \cite{edge-join,star-join,twin-twig,seed,wco-join,empty-headed,graphflow}. However, as indicated in a recent experimental work \cite{patmat-exp}, the performance of an execution plan in distributed subgraph enumeration is strongly influenced by the query, the data graph, and the hardware configurations (i.e. CPU, RAM, network), making it considerably difficult to apply the best execution plan. As a result, we design \page to be generic to accept arbitrary plan. In this subsection, we discuss existing execution plans and demonstrate how they can be represented in \page using the above operators. 
The computation frameworks of existing works\footnote{Note that \cite{crystaljoin} is an orthogonal work that proposes the compression technique, which can be applied to each framework to improve the performance \cite{patmat-exp}. We do not independently discuss it in this paper.} can be categorized via their execution plans. There are three main types of execution plans, namely binary join plan (\bj) \cite{edge-join,star-join,twin-twig,seed,psgl}, worst-case optimal plan (\wco) \cite{wco-join,Ngo-join}, and hybrid plan (\hybrid) \cite{empty-headed,graphflow}. Here, \bj involves only binary joins, \wco uses only extend operations, and \hybrid mixes both operations. All existing works adopt either directly the aforementioned plans, or their variances. We present example plans in \reffig{plans}.  
% A execution plan can be represented by a directed tree, where the node denotes the operators and the edges in between stand for the data stream. 
%As mentioned, every valid execution plan starts with \scan and ends with \sink. According to \cite{graphflow, empty-headed}, we categorize existing plans into 
%binary join plan (\bj) \cite{edge-join,star-join,twin-twig,seed,psgl}, worst-case optimal plan (\wco) \cite{wco-join,Ngo-join} and hybrid plan (\hybrid) \cite{empty-headed,graphflow}. Here, \bj involves only binary joins, \wco uses only extend operation, and \hybrid mixes both operations.

\begin{figure*}%[h]
    \centering
    \includegraphics[width=\textwidth]{figures/plans.pdf}
    \caption{Example execution plans. (Top-level subgraphs are the query graphs.)}
    \label{fig:plans}
    \vspace*{-\baselineskip}
\end{figure*}

\stitle{\bj.} By representing the query vertices as attributes and edges in the data graph as relational table, subgraph enumeration can be expressed as a series of binary joins of the edge relations (\edgejoin). For example, a triangle query can be solved by the join 
$$
\mathbb{R}(\triangle(v_1,v_2,v_3)) = E(v_1,v_2) \Join E(v_1,v_3) \Join E(v_2,v_3) ,
$$
where $E(x, y)$ refers to the edge table of the data graph, with $x, y$ as the attributes.

%Binary joins have been well studied in database research and shown to be efficient in many queries \cite{empty-headed,seed}. \edgejoin \cite{edge-join} utilizes the idea of distributed joins to compute the results of a given query. 
% As highlighted (\textcircled{1}) in \reffig{plans}, a distributed join in \page can be constructed by using \exchange-\buffer-\join. \exchange shuffles the intermediate results with the same join key to the same machine, while \buffer then buffers incoming stream in memory or on the disk. The steps are done for both the left and right streams which will be joined by a \join operator. For simplicity, we refer to an \exchange-\buffer-\join as a \emph{buffered distributed join} (\bdjoin). 
%We recursively divide the partial queries on the left and right of a join operation into \emph{sub-plan}s. Sub-plans below a \join must be fully computed before the join operation can be executed to make sure there is no missing result (\refsec{join}). 
% The reason why \buffer{s} are inserted before \join{s} is to prevent the memory from being overflowed by the intermediate results of any sub-plans; however, the presence of \buffer is optional.

\edgejoin renders numerous intermediate results, therefore \starjoin \cite{star-join} and \ttjoin \cite{twin-twig} were proposed employing the decompose-and-join paradigm. They firstly decompose the query into a set of join units such that each join unit can be enumerated independently in each partition, and then use a series of binary joins to combine the final results. \starjoin uses star as the join unit, while \ttjoin uses TwinTwig (an edge or intersection of two edges). An example of the execution plan for \starjoin is shown in \reffig{plans}a.

\stitle{\wco.} Binary joins can potentially be sub-optimal \cite{wco-thm1,wco-thm2}. \wco \cite{Ngo-join,wco-join}, on the other hand, matches the query graph one vertex at a time in a predefined order. Given a query graph $q$ and the matching order $V_q=\{v_1,v_2,\dots,v_n\}$, the plan starts from an empty set, and computes the matches of $\{v_1,\dots,v_i\}$ in the $i^{\mathrm{th}}$ round. Let a partial match after the $i^{\mathrm{th}}$ round be $p=\{u_{k_1}, u_{k_2}, \ldots, u_{k_i}\}$ for $i\leq n$, \wco expands the results in $(i+1)^{\mathrm{th}}$ round by matching $v_{i+1}$ with $u_{k_{i+1}}$ for $p$ if and only if $\forall_{1\leq j\leq i}(v_j,v_{i+1})\in E_q, (u_{k_j},u_{k_{i+1}})\in E_G$. The candidate set of $v_{i+1}$, denoted as $\mathbb{C}(v_{i+1})$ can be computed by the intersection
\begin{equation}
    \small
    \label{eq:wco}
    \mathbb{C}(v_{i + 1}) = \bigcap_{\forall_{1 \leq j \leq i} \land (v_j, v_{i + 1}) \in E_q} \mathcal{N}_G(u_{k_j}). 
\end{equation}

\page efficiently implements \wco by applying consecutive \extend operators as in the example of \reffig{plans}b. 
As mentioned (\refsec{opt}), we implement \extend via the pull-based scheme. Thus, \page can also derive the computation of existing pull-based algorithms using the \extend operators. Specifically, \rads expands the query with a star in each round and sends edge verification requests to remote machines to filter the intermediate results from such star-like expansion. This can be simply implemented as \extend-and-filter, that is firstly using \extend to extend one more vertex and then check whether the extended vertex is the specific existing vertex as highlighted (\textcircled{1}) in \reffig{plans}f. While pulling all required data locally, \benu actually adopts a sequential subgraph isomorphism algorithm \cite{ullmann}. The main idea of the algorithm is, 1) to match the query vertices along with the depth-first-search (DFS) tree, which is equivalent to extending the unmatched query vertices; 2) to check the connections between the current visited vertex and the already-matched vertices, which is equivalent to the intersection procedure in \extend. Therefore, \benu can also be supported by \page. % Although the sequential algorithm may use depth-first search (DFS), however, that can be simulated by \page's dynamic batching technique (\refsec{batch}).

\stitle{\hybrid.} \hybrid takes advantages of both \bj and \wco by combining them. \eh \cite{empty-headed} is a single-machine system which uses the \hybrid with minimum-width \emph{generalized hypertree decomposition} \cite{GHD1,GHD2}. It decomposes the query graph into sub-queries, evaluates each sub-query using a \wco, and uses a sequence of binary joins to assemble the final results. The execution plan of such system can be easily distributed and represented in \page as the example showing in \reffig{plans}c. %GraphFlow \cite{graphflow} is another single-machine system that generates hybrid execution plans based on cost estimations. Hence, the execution plan of GraphFlow for the same query may differ form different data graphs.

\seed \cite{seed} originally belongs to \bj, which uses TwinTwig and clique (a complete graph) as its join units. It indexes all triangles in the data graph to realize computing cliques on each machine. \page is designed not to depend on any indexing on storage, we can, on the other hand, uses \wco to compute the cliques, which makes \seed represented as a hybrid plan in \page. \seed adopts the optimality-guaranteed bushy join \cite{bushy-join} that dominates \edgejoin, \starjoin, and \ttjoin \cite{patmat-exp,seed}.
\reffig{plans}d illustrates a \seed execution plan. 

%Note that the execution plans generated by different algorithms may be same for certain queries. For instance, the plans of \seed and \eh are identical for the query graph shown in \reffig{plans}e. Moreover, we can make use of \clone in this example to reduce redundant computation of enumerating the same triangle.

% \vspace*{-5em}

\stitle{Plan Selection.} In \page, we select the 
% best-possible 
execution plan from \bj \cite{seed}, \wco \cite{wco-join} and \hybrid \cite{empty-headed}, that produces the smallest sum of worst-case optimal (AGM) bounds \cite{AGM} of the intermediate results.
% for \page as follows. We first compute \bj \cite{seed}, \wco \cite{wco-join} and \hybrid \cite{empty-headed}, and use the plan that produces the smallest worst-case optimal (AGM) bound \cite{AGM} of the intermediate results. 
Tie is broken by prioritising the plan with more pull-based \extend operators. As an interesting future work, we will target more sophisticated graph analytical workload on property graph model \cite{neo4j}, in which a cost-based optimiser such as \cite{graphflow, graphflow-demo} will be further investigated.

\comment{
\begin{remark}
As indicated in a recent experimental work \cite{patmat-exp}, the performance of an execution plan in distributed subgraph enumeration is strongly influenced by the query, the data graph, and the hardware configurations (i.e. CPU, RAM, network), making it considerably difficult to derive the best execution plan. We compute the execution plan as follows.  

A cost-based optimiser will facilitate the derivation of better execution plan, as a common practice in graph databases such as Neo4j \cite{neo4j} and GraphFlow \cite{graphflow-demo}. In this paper, we rather focus on proposing the computing engine of distributed subgraph enumeration, and leave such an optimiser as a future work.
%, when we will consider richer semantics with labels and properties.  %has been frequently applied to DBMS \cite{query-opt1,query-opt2,logicblox} to automatically derive the execution plan for a query. Such optimisers are also adopted by graph databases such as Neo4j \cite{neo4j} and GraphFlow \cite{graphflow-demo} for better query execution. In this paper, we rather focus on proposing the computing infrastructure of distributed subgraph enumeration, and leave the cost-based optimiser as a future work, where we will further consider a data graph with rich labels and properties.
\end{remark}
}

==> contents/introduction-old.tex <==
\section{Introduction}
\label{sec:intro}

The problem of subgraph enumeration is to find all subgraph instances of a data graph $G$ that are isomorphic to a query graph $q$. As a fundamental problem in graph analytics and a core operation of graph databases such as Neo4j \cite{neo4j} and RDF engines \cite{gstore}, it has been used in a wide spectrum of applications \cite{chemical,protein,www,biomolecular,motif,recommend,GPAR,net-analy}.
% In this paper, we assume that the graph is undirected and unlabeled\footnote{Our implementation can seamlessly support directed and labeled graph.}. 
With the massive growth in graph size nowadays \cite{ubiquity} and the NP-hardness \cite{np-complete} of subgraph enumeration, researchers have devoted a lot of efforts into developing efficient and scalable algorithms in the distributed context \cite{crystaljoin,wco-join,twin-twig,edge-join,star-join,seed,psgl,RADS,BENU,multiway-join}. Specifically, we categorize these algorithms into join-based scheme and pull-based scheme.

\stitle{Join-based scheme.} % By representing query vertices as attributes and data vertices as tuples in the relation table, subgraph enumeration can be expressed as the join problem. 
%Subgraph enumeration can be conducted by joins. 
Join-based algorithms \cite{crystaljoin,wco-join,twin-twig,edge-join,star-join,seed} adopt distributed join to compute matches of a given query. It can be further classified into primarily binary join (\eaat) and worst-case optimal join (\vaat). \eaat \cite{twin-twig,seed,edge-join,star-join,crystaljoin} decomposes the query graph into a set of join units whose matches can be computed independently in each partition, and applies a series of binary joins to assemble the final results. \vaat-based algorithm \bigjoin \cite{wco-join} extends the query graph one vertex at a time by intersecting the neighbors of all its connected vertices, following Ngo's join algorithms \cite{Ngo-join} for worst-case optimality \cite{AGM}. Join-based algorithms usually encounter large volume of communication when shuffling the intermediate results in the cluster.% during the distributed join phase.

\stitle{Pull-based scheme.} Pull-based algorithms aim at reducing the size of communication for join-based algorithms. %A first solution, \multiwayjoin \cite{multiway-join}, maintains graph partitioning with duplication so that we can process subgraph matching independently in each partition without missing results. This solution has been shown \cite{patmat-exp} to scale poorly, with each partition almost carrying a whole share of the data graph. 
%The typical solution utilizes the idea of "pull-and-caching" \cite{BENU,RADS}, that is to process subgraph matching using the serial backtracking algorithm \cite{comparison} as if it is in one single machine, while pulling unpresented data from remote machine during the process and properly caching it for further reuse.
\benu \cite{BENU} stores the data graph in a distributed key-value database 
% such as HBase \cite{hbase} 
and uses concurrent cache in each machine to cache recently accessed vertices. Then it processes subgraph matching using the serial backtracking algorithm \cite{comparison} as if it is in one single machine. %leaving the communication entirely to the distributed key-value store. 
% The performance of \benu is therefore highly dependent on the chosen key-value database.
\rads \cite{RADS} is another pull-based algorithm that employs a multi-round expand-and-filter paradigm. It expands a pivot vertex with a star (a tree of depth $1$) in each round and verifies cross and sibling edges to filter out unmatched results using edge verification index. The intermediate results of matching stars can be dramatically large \cite{twin-twig}. 
For example, if the query graph contains a 3-star (a star with 3 leaves), it produces over $7$ \emph{trillion} results on the largest-degree vertex of the \dtuk dataset (\reftable{data}).
% a vertex with degree $10,000$ can have over $O(10^{12})$ matches when matching with a $3$-star. 
In addition, the idea of postponing edge verification after expanding further leads to enormous unpromising intermediate results \cite{DAF}. 
% Note that \rads also proposed an optimization of single-machine enumeration that identifies locally available matches in advance and launch an early round to compute them without any communication.
% This optimization can be orthogonally applied to other algorithms as well. 
% However, since the number of local matches heavily relies on the quality of graph partitioning and computing high-quality partitions for large graphs is particularly challenging \cite{partition1,partition2}, the effect of this optimization is often very limited. 
% Following previous works of large-scale distributed subgraph matching \cite{patmat-exp} and to reduce overheads of our system \cite{gemini}, we consider a simple hash partition in this paper.


\comment{
The state-of-the-arts of distributed subgraph enumeration, except \rads, are all \emph{algorithmic} works. They are developed on either existing big-data engines (e.g. Hadoop for \seed, Timely dataflow engine for \bigjoin) or distributed key-value store (e.g. Cassandra for \benu), which has exposed some drawbacks: (1) The performance of subgraph enumeration is often bound to the limitations of the based infrastructures. For algorithms based on big-data engines (all join-based algorithms), it is infeasible to leverage the pull-based mechanism to reduce the communication cost where possible. \benu does benefit from pulling data from a distributed key-value store to reduce the communication volume, which, however, does not contribute to reducing the communication time of \benu, mainly due to the low throughput of the key-value store; (2) The exponential nature of subgraph enumeration can often result in serious memory crisis, especially for the join-based algorithms that attempt to materialize the intermediate results for join. Existing big-data engines require the developer to concern about memory usage while implementing the algorithm. Ad-hoc solution like static batching that limits the number of initial matched (pivot) vertices/edges \cite{wco-join} does not have guarantee and can often fail to bound memory usage for arbitrary query and data graph (\refsec{experiment}); (3) The algorithms are all tightly coupled with certain execution plan, which may miss the chance of an optimal execution. For example, \eaat algorithms adopt only binary joins, and \vaat algorithms are based on worst-case optimal join \cite{Ngo-join}, while neither \eaat nor \vaat plans are guaranteed to be optimal \cite{patmat-exp,match-survey, graphflow, empty-headed}.  %Ad-hoc solution such as static batching \cite{wco-join} that limits the number of initial matched (pivot) vertices/edges is typically adopted, while the 

%Comparatively, \benu stores the data graph in a distributed key-value store\footnote{We use Cassandra as recommended by the authors to provide better throughput.}, and pull and cache remote data as needed. Although with substantially smaller communication volume, this design does not contribute to \benu's lower communication time, mainly due to the low throughput of the key-value store, and massive contentions and data copies while accessing local cache. 

  %while the high irregularity of graph access pattern makes it impossible to determine a proper initial value. %For example, given a query graph of 4-path (a consecutive connection of 4 edges) and a data graph where each vertex has a degree of 1000, the query can produce 1,000,000,000,000 results from one single vertex.

%To show this, we have conducted an initial experiment by running the square query ($\bm{\square}$) over the \dtlj graph using representative algorithms\footnote{Two best-performed join-based algorithms \seed and \bigjoin \cite{patmat-exp}, and two pull-based algorithms \benu and \rads}, which is a popular task for benchmarking subgraph enumeration \cite{patmat-exp, wco-join, RADS, BENU}. The results are presented in \reftable{intro_exp}.

%Firstly, 

%Detailed implementations and setups can be found in \refsec{exp} and 

%Firstly, while existing big-data engines lack in the support of pull-based communication, it is infeasible to leverage the pull-based scheme to reduce the communication cost. It is clear from \reftable{intro_exp} that the join-based algorithms, \seed and \bigjoin, produce a larger volume of communication than the pull-based alternatives. A naive solution developed by \benu is to store the data graph in a distributed key-value store, and pull and cache remote data as needed. Although with substantially smaller communication volume, this design does not contribute to \benu's lower communication time than \bigjoin as a join-based algorithm. A deeper investigation reveals that \benu spends a large portion of time accessing the cache due to enormous \emph{data contentions} and \emph{memory copies}. 

%Secondly, the exponential nature of subgraph enumeration can often result in serious memory crisis. Observe that all existing algorithms (except \benu, will discuss later) in \reftable{intro_exp} consume much more memory than the data graph itself (2GB for \dtlj). Existing big-data engines require the developer to concern about memory usage while implementing the algorithm. Ad-hoc solutions such as static batching \cite{wco-join,RADS} that limits the number of initial matched vertices/edges are typically adopted, while the memory consumption still remains at a high level.


%Thirdly, all existing algorithms are tightly coupled with certain execution plan, which may miss the chance of an optimal execution. For example, \eaat algorithms adopt only binary joins, and \vaat algorithms are based on worst-case optimal join \cite{Ngo-join}, while neither \eaat nor \vaat plans are guaranteed to be optimal \cite{patmat-exp,match-survey, graphflow, empty-headed}.
%To better implement the pull-based scheme, \rads employs a multi-round of ``star-expand-and-filter'' process, which is essentially a \starjoin plan \cite{twin-twig}. As shown in \cite{patmat-exp,match-survey, graphflow, empty-headed}, none of these algorithmic works are guaranteed to adopt the optimal execution plan for arbitrary query and data graph. 

%most algorithms are developed based on existing big-data engines (e.g. Hadoop \cite{hadoop} and Timely dataflow engine \cite{naiad}). While these engines lack in the support of pull-based communication, it is infeasible to leverage the pull-based scheme to reduce the communication cost. It is clear from \reftable{intro_exp} that the join-based algorithms, \seed and \bigjoin, produce a larger volume of communication than the pull-based algorithms. Additionally, the exponential nature of subgraph enumeration can often result in serious memory crisis. Observe that all existing algorithms (except \benu, will discuss later) in \reftable{intro_exp} consume much more memory than the data graph itself (2GB for \dtlj). Existing big-data engines require the developer to concern about memory usage while implementing the algorithm. Ad-hoc solutions such as static batching \cite{wco-join,RADS} that limits the number of initial matched vertices/edges are typically adopted, while the memory utilization still remains at a high level.

 %For square query specifically, it will have to materialize all paths of length 3 to verify the matching of last edge. This execution plan is sub-optimal to the worst-case optimal join, which leads to long computation time and high memory consumption.
%To facilitate pull-based communication, \rads employs a multi-round expand-and-filter paradigm to expand a pivot vertex with a star (a tree of depth $1$) in each round and verifies cross and sibling edges to filter out unmatched results using edge verification index. For this query, the execution plans materialize all matchings of a 3-path ($\bm{\sqcap}$) in order to verify the last edge, where the data graph has more than $200$ billion eligible $3$-paths. This leads to a long computation time and high memory consumption for \rads as can be observed. However, it is not able to select a better execution plan (e.g. \bigjoin's plan) for \rads to take the advantages of pull-based communication. As shown both experimentally \cite{patmat-exp,match-survey} and theoretically \cite{graphflow,empty-headed}, none of these algorithmic works are guaranteed to adopt the best execution plan for arbitrary query and data graph.
%The optimal execution plan can even be a mixture of \eaat and \vaat \cite{graphflow,empty-headed}.


%Thirdly, the exponential nature of subgraph enumeration can result in serious memory crisis. Observe that all existing algorithms except \benu in \reftable{intro_exp} consume much more memory than the data graph itself (2GB for \dtlj). 

Motivated by the above drawbacks, \rads has developed its own computation engine with a pulling design and the memory controlling strategy called region group. The main idea is to extend an intermediate results with a star (a tree of depth 1). Observe that the stars rooted on a vertex can be enumerated from its adjacent vertices (neighbors) \cite{twin-twig}. Instead of shuffling the intermediate results, the extension can hence be processed by pulling a remote vertex with its neighbors and then computing locally. However, to facilitate such a pulling design, \rads is coupled with a certain execution plan that is essentially a \starjoin \cite{star-join}, which has already been shown to be sub-optimal \cite{seed, wco-join}. In addition, the region-group strategy in \rads is still a variant of the static batching technique without guarantee. As a result, we have observed \rads's relatively poor performance with considerable memory consumption in the experiment (\refsec{experiment}).

In summary, the efficient and scalable execution of subgraph enumeration requires the \emph{systematic} considerations of (1) a \emph{generic execution plan} decoupled from the runtime; (2) a novel \emph{hybrid computation engine} that supports both pulling data and shuffling data\footnote{Although pulling mechanism is often more communication-efficient, but a purely pulling design, for examples \rads, may limit the execution to a possibly sub-optimal plan.} efficiently as required; and (3) an \emph{efficient, memory-bounded execution} with theoretical guarantee.
}


\stitle{Motivations.} %Join-based algorithms can generate a huge number of intermediate results during distributed joins that are usually even larger than the data graph itself. 
% For instance, there are more than 34 billion triangles (a core structure of join-based algorithms) in Twitter's social graph, which is about 30 times larger than the number of edges in the graph \cite{triangle}. 
%The intermediate results are shuffled across machines, leading to high volume of communication. 
Join-based algorithms can shuffle enormous intermediate results, leading to huge communication cost. Naturally, the pull-based algorithms should have the obvious advantage with much reduced communication cost. However, as our initial experiments revealed, the state-of-the-art pull-based algorithms, namely \benu and \rads, can often be outperformed by join-based algorithms, for example \bigjoin, in term of execution time. Detailed implementations of these algorithms can be found in \refsec{exp}.
%We adopt the implementation for the join-based algorithms in \cite{patmat-exp}. For fairness, we implement \benu an \rads in Rust using our best effort as well as email communications with the authors. 
We run the square query ($\bm{\square}$) over the \dtlj graph (\reftable{data}), which is a popular data graph for benchmarking subgraph enumeration \cite{patmat-exp, wco-join, RADS, BENU}. The results are in \reftable{intro_exp}, including the total time ($T$), computation time ($T_R$), communication time ($T_C = T - T_R$) \cite{patmat-exp}, the total size of data transferred over the network ($C$), and the peak memory usage ($M$) among all machines.  %We measure total time ($T$) and computation time ($T_R$), and let  communication time $T_C = T - T_R$ according to \cite{patmat-exp}. We also report the total size of data transferred over the network ($C$), and the maximum memory usage ($M$) among all machines. The results are in \reftable{intro_exp}  %we measure computation time by timing the functions that conduct the de-facto computation, and take computation time off the total time as the communication time.

\begin{table}[]
\caption{Results of running a square query over the \dtlj graph in a local 10-machine cluster (\refsec{exp}).}%, conducted on a cluster with 10 machines, 4 cores each machine, connected via a 10Gbps network.}
\label{tab:intro_exp}
\small
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
%Scheme & Algorithm & \begin{tabular}[c]{@{}c@{}}Total\\ Time(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Comp.\\ Time(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Comm. \\ Time(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}Total\\ Comm.\end{tabular} \\ \hline
Scheme & Algorithm & \begin{tabular}[c]{@{}c@{}}$T$(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$T_R$(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$T_C$(s)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$C$(GB)\end{tabular} & \begin{tabular}[c]{@{}c@{}}$M$(GB)\end{tabular}\\ \hline
\multirow{2}{*}{Pull-based} & \benu & $4472.7$ & $3773.1$ & $699.6$ &  $76.5$ & $1.3$ \\ \cline{2-7} 
 & \rads & $2643.8$ & $2478.7$ & $165.1$  & $452.7$ & $19.2$ \\ \hline
Join-based & \bigjoin & $195.9$ & $122.1$ & $73.8$ & $534.5$ & $14.3$ \\ \hline\hline
\textbf{Hybrid} & \begin{tabular}[c]{@{}c@{}}\page\end{tabular} & $52.7$ & $52.3$ & $0.4$ & $2.4$ & $2.2$ \\ \hline
\end{tabular}
\vspace*{-\baselineskip}
\end{table}

% \footnotetext[1]{\page runs the worst-case optimal plan in this experiment.}

\benu and \rads transfer less data across the network than \bigjoin, but do not demonstrate reduced communication time. For \benu, %communication is handled by the key-value database. 
we have used the high-performance key-value database Cassandra \cite{cassandra} to store the data graph as recommended by the authors of \cite{BENU}. However, %the performance is poor due to %still heavily limited by the 
due to the low throughput of the key-value database, the communication gain is overturned by waiting data from the key-value database. %As we observed in the above experiment, the database takes a large portion of the overall resources in the cluster. 
For \rads, pull requests are sent one by one that cannot fully utilize the network bandwidth, which adds significant overhead to communication. In addition, we can observe that \rads also produces very large communication volume, because of the enormous edge verification requests. %and The reason why \rads has higher communication volume than \benu is because its large edge verification requests, which are not cached.

For the computation part, the computation time of \rads is long because of its poor execution plan, which must materialize all matchings of a 3-path ($\bm{\sqcap}$) in order to verify the last edge. In the initial experiment, the data graph has more than $200$ billion eligible $3$-paths, which makes \rads extremely time-consuming and memory-intensive. \bigjoin, however, computes this query by enumerating all 2-stars and intersecting the neighbors of the two leaf vertices, resulted in much less intermediate results, and hence better performance. For \benu, vertices can be obtained from the cache during computation. However, getting vertices from the shared concurrent cache is expensive, due to the interplay of CPU instructions, memory copies and exclusive lock. We observe that about $90\%$ of the computing time of \benu is spent on getting vertices from the cache.
More critically, \benu triggers a vast number of expensive recursive calls that may involve pulling remote data when doing backtracking using depth-first search (DFS), which results in low CPU utilization.  %, especially when each recursive call may have to pull the remote data, resulting in low CPU utilization. 

We summarize the issues of existing pull-based algorithms as follows.

% \vspace*{-\baselineskip}

% [leftmargin=0cm,itemindent=.5cm,labelwidth=\itemindent,labelsep=0cm,align=left]
\begin{enumerate} [leftmargin=*] %[label=Issue \arabic*, wide=0pt, leftmargin=0.5cm]
  \item \textit{Poor Execution Plan.} A poor execution plan (e.g. \rads) can cause the program to run overtime or out of memory due to the production of enormous intermediate results.
 % Furthermore, as stated in a recent experimental work \cite{patmat-exp}, the performance of an execution plan is jointly affected by the query, the data graph and even the hardware configurations.
  % , and none of existing plans (e.g. worst-case optimal, binary join) are guaranteed to perform the best at all circumstances. However, 
  All existing distributed algorithms are coupled with one certain execution plan, missing the opportunities of trying out other existing plans.

  \item \textit{Inefficient Computation.} Existing pull-based algorithms can have severe bottleneck in computation due to the inefficient cache design and computation paradigm (e.g. DFS in \benu). %, and thus inefficient computation.
  
%   Existing pull-based algorithm (i.e. \benu) can have severe bottleneck while triggering a vast number of expensive recursive calls when doing backtracking using depth-first search (DFS), especially when each recursive call may have to pull the remote data. In addition, DFS algorithms are hard to parallelize, resulting in low CPU utilization as illustrated and thus inefficient computation. More importantly, it shares a cache (e.g. LRU, LFU) over all workers in a single machine to increase cache hits and reduce network access, which suffers from significant locking on cache. This is because locks must be imposed on the shared cache to ensure consistence and then each read or write operation will trigger the lock on cache. We noticed that about $90\%$ of the computing time of \benu are spent on getting vertices from the cache, which significantly slows down the program and increases CPU instructions.
 
%   \item \underline{Significant Locking on Cache.} Current pull-based algorithms share a cache (LRU) over all workers in a single machine to increase cache hits and reduce network access.
% Hence, locks must be imposed on the shared cache to ensure consistence. Read and write operations will trigger lock operations on the cache, which significantly slows down the program and increases CPU instructions.
\end{enumerate}
  
Moreover, we have identified another two general issues of distributed subgraph enumeration.

% \vspace*{-.3em}

\begin{enumerate}[start=3, leftmargin=*]% label=Issue \arabic*, wide=0pt, leftmargin=0.5cm]
    \item \textit{Memory Crisis.} %While running pure DFS algorithms in distributed environment leads to low CPU utilization, 
    %\todo{Try to use communication instead of memory.}
    While DFS-based paradigm can bound memory usage, it often leads to low CPU utilization, e.g. \benu. Most existing algorithms (\rads and all join-based algorithms) rather use a breadth-first-search (BFS) -based paradigm, requiring large amount of memory to maintain the intermediate results, as can be seen in \reftable{intro_exp}. %Techniques such as batching \cite{patmat-exp, wco-join} and region group \cite{RADS}
    %As we can see in \reftable{intro_exp}, all solutions except \benu uses large amount of memory (larger than maintaining the data graph itself). The low memory usage of \benu comes from the DFS-based computation paradigm. % current solutions (especially join-based algorithms) % approaches of breath-first search (BFS) algorithms (all join-based algorithms)
    %are unable to control the memory usage well. 
    %However, due to low CPU utilization of DFS-based paradigm, most \Specific techniques such as batching \cite{patmat-exp,wco-join} are applied 
    % of region group \cite{RADS}
    % splitting the first vertex/edge matched into small groups 
    %have been used to reduce memory consumption. However, even though the size of the initial batching/region group is small, it can expand exponentially at any stage of the computation, making the program run out of memory. 
    % For the same reason, in the pull-based algorithms, one cannot expect replacing the DFS component with BFS-style routine in the hope of resolving inefficient computation for all.
    
    \item \textit{Poor Load Balancing.} All existing solutions typically distribute load based on the firstly matched vertex/edge, which easily results in load skew. This is likely to happen especially in real-world power-law graphs \cite{power-law-1,power-law-2} where a super vertex (a vertex of extremely large degree) can produce significantly higher load than all other vertices. 
\end{enumerate}

\stitle{Contributions.} It is challenging to solve the aforementioned problems of distributed subgraph enumeration, which requires a systematic work of refactoring the architecture of subgraph enumeration. 
%, with a novel cache design and fine-grained scheduling techniques. 
In this paper, we present \page, an efficient and scalable join/pull-\textbf{H}ybrid s\textbf{U}b\textbf{G}raph \textbf{E}numeration engine.%, and uses much less memory for the query in \reftable{intro_exp}.

\page is efficient in both communication and computation. For communication, \page prioritises pull-based scheme to avoid the obvious limitation of distributed joins that suffocates in shuffling enormous intermediate results. It does not depend on any external storage (e.g. distributed key-value store) and can effectively aggregate pull requests to further reduce communication size and improve network utilization. As indicated in the above example, \page achieves the smallest communication size of $2.4$GB.
% among all solutions. 

For computation, \page adopts a novel execution mode together with a fine-grained dynamic scheduler to fully utilize the parallel computation while bouding the memory usage. \page also supports a hybrid scheme that mixes join-based and pull-based scheme, in case that the resulted execution plan leads to a better distributed runtime \cite{empty-headed,graphflow,patmat-exp}. As a result, \page offers a much better query performance, with 84$\times$, 50$\times$ and 3.7$\times$ gain than \benu, \rads and \bigjoin in \reftable{intro_exp}, respectively. Meanwhile, \page is also memory-efficient, with memory usage much lower than \rads and \bigjoin, and close to the DFS-based solution \benu.  
% \todo{discuss the memory usage.} %Furthermore, \page is in-general memory-efficient, which may not be significant for the motivating example that queries $q_1$ on the relatively small dataset LiveJournal. However, we have observed many cases in the experiment (\refsec{exp}) that \page can complete the computation while all state-of-the-arts are out of memory.

We design \page to be generic to support different execution plans, and has the potential of selecting the best-possible plans. In addition, all existing distributed subgraph enumeration algorithms can not only be effortlessly represented in \page, but also executed with immediate speed up and bounded memory consumption due to our systematic contributions. Take \vaat as an example, while being executed in \page\footnote{\page runs the worst-case optimal plan in the initial experiment.}, it outperforms the existing \vaat-based algorithm \bigjoin by over 3.7$\times$ in \reftable{intro_exp}, while using $6.5\times$ less memory. 

%As a result, all existing distributed subgraph enumeration algorithms can be effortlessly represented in \page, and executed with automatic speed up and bounded memory consumption. Take \vaat as an example, while being executed in \page (denoted as \pagewco), it outperforms the existing \vaat-based algorithm \bigjoin by over 3.7$\times$, and uses much less memory for the query in \reftable{intro_exp}. %In addition, \page addresses the problems of inefficient computation and poor load balancing, resulting a much better query performance (84$\times$, 50$\times$ and 3.7$\times$ than \benu, \rads and \bigjoin in \reftable{intro_exp}). 

We summarize the main contributions of this paper as follows.

% \todo{Where is memory, because you did mention memory crisis}  
% (\todo{I think this paragraph is very long and useless }) 
%\page is efficient in both communication and computation. For communication, \page prioritises pull-based scheme to avoid the obvious limitation of distributed joins that suffocates in shuffling enormous intermediate results. It does not depend on any external storage (e.g. distributed key-value store) and can effectively aggregate pull requests to further reduce communication size and improve network utilization. As indicated in the above example, \page achieves the smallest communication size of $2.4$GB among all solutions. While for computation, \page uses a novel execution mode together with a fine-grained dynamic scheduler to increases the computation efficiency and degree of parallelism. \page also supports a hybrid scheme that mixing join-based and pull-based scheme, in case the resulted execution plan leads to a better distributed runtime \cite{empty-headed,graphflow,patmat-exp}. The main contributions of this paper are:

% As a hybrid scheme, we also design \page to support join in the execution, in case that there is better distributed runtime while leveraging the join operation \cite{empty-headed,graphflow,patmat-exp}. 
% To summary, \page is 
% 1) generic that allows user to plugin different execution plans that may include joins; 
% 2) CPU- and memory-efficient that outperforms the state-of-the-arts by up to xx orders of magnitude; 
% 3) much more communication-friendly than the pure join-based algorithms. 
% A quick comparison between \page and the state-of-the-arts is listed in \reftable{summary}, with respect to computation efficiency (Comp.), communication cost (Comm.), and memory usage (Mem.).

% \vspace{-.4\baselineskip}

\begin{enumerate}[leftmargin=*]
  \item \textit{A generic hybrid engine for distributed subgraph enumeration.} To solve issue 1, \page is designed to be index-free and generic to accept arbitrary execution plans including worst-case optimal plan \cite{wco-join}, binary join plan \cite{edge-join,star-join,twin-twig,seed,crystaljoin} and hybrid execution plan \cite{graphflow,empty-headed}, etc. It improves the performance of all existing algorithms and supports a seamless mixture between pull-based scheme and join-based scheme.%, resulting in better execution plan in some use cases.
  
  \item \textit{A two-stage execution mode with lock-free and zero-copy cache design.} For issue 2, we propose a novel two-stage execution mode to efficiently pull remote data while keeping all computation process in parallel. With this computation model, we designed a concurrent cache structure that is lock-free and zero-copy which greatly increases the performance of pull-based distributed subgraph enumeration scheme.
  
  \item \textit{A hybrid BFS-DFS dynamic scheduler.} To solve issue 3 while maximizing resource utilization, we introduce a hybrid BFS-DFS dynamic scheduler. It adopts BFS-style scheduling whenever it is possible and switches to DFS-style scheduling if the memory is insufficient. % to consume the intermediate results.
  A threshold can be set for memory usage enabling the program to be run within bounded memory under full CPU utilization.
  
  \item \textit{Operator level intra- and inter-machine work stealing mechanism.} For issue 4, \page adopts work stealing at operator level both intra- and inter-machine to achieve nearly perfect load balancing in real-world skewed graphs.
  
  \item \textit{In-depth experiments.} We conduct extensive experiments on 7 real world graphs.  Results show that \page outperforms previously best pull-based algorithm by up to $113\times$; and the best join-based algorithm by up to $7.8\times$, with considerably much less communication.
\end{enumerate}

\stitle{Paper Organization.} The rest of this paper is organized as follows. \refsec{pre} introduces preliminaries. \refsec{framework} presents the computation framework of \page. In \refsec{impl}, we discuss implementation details of \page. In \refsec{schedule}, we presents how an execution plan is scheduled in \page. Experimental evaluations are presented in \refsec{exp}, followed by related work in \refsec{related}. Finally, we conclude the paper in \refsec{conclusion}.
